CAMELTrack: Context-Aware Multi-cue ExpLoitation for Online Multi-Object Tracking

Online multi-object tracking has been recently dominated by tracking-by-detection (TbD) methods, where recent advances rely on increasingly sophisticated heuristics for tracklet representation, feature fusion, and multi-stage matching. The key strength of TbD lies in its modular design, enabling the integration of specialized off-the-shelf models like motion predictors and re-identification. However, the extensive usage of human-crafted rules for temporal associations makes these methods inherently limited in their ability to capture the complex interplay between various tracking cues. In this work, we introduce CAMEL, a novel association module for Context-Aware Multi-Cue ExpLoitation, that learns resilient association strategies directly from data, breaking free from hand-crafted heuristics while maintaining TbD's valuable modularity. At its core, CAMEL employs two transformer-based modules and relies on a novel association-centric training scheme to effectively model the complex interactions between tracked targets and their various association cues. Unlike end-to-end detection-by-tracking approaches, our method remains lightweight and fast to train while being able to leverage external off-the-shelf models. Our proposed online tracking pipeline, CAMELTrack, achieves state-of-the-art performance on multiple tracking benchmarks. Our code is available at https://github.com/TrackingLaboratory/CAMELTrack.

==> figures/related_work_taxonomy.tex <==



\begin{figure}[t]
    \centering
    \definecolor{darkgreen}{RGB}{0,128,0}
    \definecolor{darkred}{RGB}{139,0,0}
    \begin{tikzpicture}[
        level 1/.style={level distance=0.5cm, sibling distance=42mm},
        level 2/.style={level distance=0.8cm, sibling distance=28mm},
        level 3/.style={level distance=1.3cm, sibling distance=20mm}, % Increased last level distance
        edge from parent/.style={draw, -latex},
        every node/.style={font=\small},
        method_purple/.style={font=\footnotesize\itshape, text=purple},
        method_black/.style={font=\footnotesize\itshape, text=black},
        result_text/.style={font=\footnotesize, align=center, text depth=0.5ex}
    ]
        \node {\textbf{Online TbD}}
        child {
            node {TbD} 
            child {
                node {Heuristic Association}
                child {
                    node[result_text] {\textit{ByteTrack}~\cite{bytetrack}, ... \\ 
                    \textcolor{darkred}{\xmark} HFA 
                    \textcolor{darkgreen}{\cmark} OM 
                    \textcolor{darkgreen}{\cmark} LC}
                }
            }
            child {
                node {Learned Association}
                child {
                    node[result_text] {\textcolor{purple}{\textit{CAMEL}} \textit{(ours)} \\ 
                    \textcolor{darkgreen}{\cmark} HFA 
                    \textcolor{darkgreen}{\cmark} OM 
                    \textcolor{darkgreen}{\cmark} LC}
                }
            }
        }
        child {
            node {DbT} 
            child {
                node {E2E}
                child {
                    node[result_text] {\textit{MOTR}~\cite{motr}, ... \\ 
                    \textcolor{darkgreen}{\cmark} HFA 
                    \textcolor{darkred}{\xmark} OM 
                    \textcolor{darkred}{\xmark} LC}
                }
            }
        };
    \end{tikzpicture}
    \caption{Hierarchy of data association methods for Online MOT. HF stands for Heuristic-Free association, OM refers to the ability to use Off-the-shelf Models, and LC denotes Low training Compute.}
    \label{fig:mot_taxonomy}
\end{figure}

==> figures/training_sample.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/assets/training-sample3.pdf}
    \caption{A training sample from our Association-centric Training scheme. Dashes and bold lines illustrate original and augmented tracklets, respectively.
    }
    \label{fig:training-sample}
\end{figure} 


